Prompting Large Language Models With the Socratic Method

This paper presents a systematic approach to using the Socratic method in developing prompt templates that effectively interact with large language models, including GPT-3. Various methods are examined, and those that yield precise answers and justifications while fostering creativity and imagination to enhance creative writing are identified. Techniques such as {\em definition}, {\em elenchus}, {\em dialectic}, {\em maieutics}, {\em generalization}, and {\em counterfactual reasoning} are discussed for their application in engineering prompt templates and their connections to inductive, deductive, and abductive reasoning. Through examples, the effectiveness of these dialogue and reasoning methods is demonstrated. An interesting observation is made that when the task's goal and user intent are conveyed to GPT-3 via ChatGPT before the start of a dialogue, the large language model seems to connect to the external context expressed in the intent and perform more effectively.

==> BackupPPromptTemplate.tex <==
\section{Prompt Template Engineering}
\label{sec:template}

Our examples with GPT-3, utilizing the ChatGPT user interface and its APIs, have revealed that utilizing the methods of definition, elenchus, dialectic, maieutics, counterfactual reasoning can effectively enhance the output's accuracy and conciseness through arguments and verification, as well as showcase guided generalization and creativity. The ongoing challenge is to generate prompt templates within an interactive setting, with each prompt being generated based on the context accumulated thus far, akin to the Socratic method of recollection.

Prompt template engineering refers to the process of designing and creating templates for providing input, or ``prompts,'' to a language model to guide its output generation. This section first discusses prompt template engineering methods for
the basic building blocks, and then integrates the the methods of definition, elenchus, maieutics, counterfactual reasoning to compose complex templates.

\subsection{Basic, One Shot Template}

Let us start with a simple one-shot template.
The work of \cite{SocraticModels-Google2022} uses a simple formulation function to generate prompt $x'$,
$x'$ = $f_{prompt}$($x$) given input $x$.

For the task of machine translation, the template may take a form “Translate from [Lan$_{from}$]: [X] to [Lan$_{to}$]: [Y],” where Lan$_{from}$ can be detected
by the prompt template or can rely on the LLM
to find out. Input $x$ consists of information to
fill slots [X] and [Lan$_{to}$].
For instance, if input $x$ is ``translate good morning to French,'' the template $x'$ is filled with the
information in $x$, and $x'$ = ``Translate from English: ``good morning'' to French: [Y].''  The empty slot [Y] is
for the LLM to return.  
Once the LLM has completed the translation task, it
replaces Y to be ``bonjour.'' In cases when LLM may return multiple responses
(e.g., when x is a word with multiple meanings without additional context), it also provides a score for each. The prompt template can decide to
output the response with the highest score, or to
send back to the LLM to produce a summarize.

There are three main design considerations when engineering a basic prompt. First, it is important to consider how to phrase the template so that it can handle different styles of user input for the same task. For example, a user may ask for a translation task to be performed by saying ``Translate x to French'' or ``What is the French translation of x?''. Second, as discussed in \cite{PromptSurvey2023}, it is important to take into account the patterns and capabilities of the partner language model (LLM) when designing the template, such as whether the LLM is left-to-right \cite{OpenAI-GPT3-2020} or masked \cite{Devlin2019BERTPO}. Third, certain tasks, such as language detection and summarization, can be performed by the template itself or by the LLM. The decision between these options should take into account factors such as cost, as using an LLM often incurs a fee, while developing a template as a client module can be done for free.

To address the first two technical challenges, one can first hand-engineer a few seed templates and then paraphrase them into an ensemble \cite{Haviv2021BERTeseLT}. We believe that the basic, one-shot formulation can always be replaced by an ensemble formulation \cite{Schick2020ExploitingCF,Peng2022ModelEI} and then learn the weights of its members for each query instance to produce the final output. Additionally, it is not necessary to conduct mining on LLMs to understand their capabilities, as an ensemble with various paraphrased prompts can find out what an LLM knows by examining which basic prompts have high weights. From those highly weighted prompts, we can infer the strengths of the LLM. 

%\noindent
%{\color{blue} Note} Experiment idea: evaluate LLMs using ensembles.

\subsection{Clarification with Method Definition}
\label{sec:template-definition}

There are computer algorithms that can already be used to recursively clarify a question, its definitions, and sub-terms' definitions. In fact, the natural language processing (NLP) community has developed a large 
number of useful methods and algorithms over the years \cite{NLP-Text-JM3}. 
One can use NLP techniques, such as dependency parsing and named-entity recognition (NER) \cite{NLPScratch2011}, to analyze the structure and meaning of a question and identify key terms and concepts. For example, 
NER can be used to extract entities in user input, such as names, locations, and organizations, and co-reference resolution can be used to understand the referred entity of a pronoun. 
Before submitting a template to an LLM, the application (e.g., a chatbot) 
that uses the template should check if all input slots are filled, 
and perform a sanity check. In the translation example, if the [Lan$_{to}$] was not provided or the specified language is not supported by the LLM, then the application should inquire the user for clarification.

Regarding mapping a natural language input to a prompt template, existing techniques of knowledge representation and reasoning can be very helpful. More specifically, ontology alignment and semantic parsing \cite{Campagna2020AFS,zhou-etal-2021-structure} can help map an NL input to a structured representation of knowledge and infer implicit concepts and relationships. These algorithms can be used to generate more precise and accurate prompts for LLMs, and to improve the effectiveness of the Socratic method in dialogue formulation \cite{DialoguewithAttention2023}. Some available tools include NLTK (Natural Language Toolkit) and spaCy for NLP\footnote{spaCy (https://spacy.io/)}, and TensorFlow for ML\footnote{TensorFlow (https://www.tensorflow.org/)}.

%\noindent
%{\color{blue} Note} Experiment idea: compare w/ and w/o.

\subsection{Verification with Method Elenchus}

The main purposes of conducting cross examination in a template are to validate the credibility of the information sources and to identify inconsistencies in the process. Cross examination is typically conducted through a multi-turn dialogue \cite{DialoguewithAttention2023}. In the context of template engineering, the goal is to formulate a productive dialogue that can be used to assess the reliability of an LLM's output.  

There are several methods that can be used to assess and strengthen the reliability of an LLM's output. 1) The first approach is to paraphrase a question in order to obtain different answers and identify inconsistencies, if they exist, in multiple answers. 2) The second method is to ask for further evidence, such as querying top-k sources of information and asking the LLM to rate the credibility of each source. This can be used to compute the reliability of the output. 3) Additionally, template engineering can be used to query an LLM for opposing views of its output, including sources and credibility, and then evaluate if a different perspective is strong.

The implementation of the first two methods for cross examination, paraphrasing a question and asking for further evidence, is readily covered by the techniques enumerated in Section~\ref{sec:template-definition}. To implement the third method of asking for different perspectives, a simple approach is to find the sentiment of the original question and then rewrite the question with an opposite sentiment. For example, if the original question is phrased in a positive tone, the prompt template can reformulate the question with a negative tone to elicit a contrasting viewpoint.
A more elaborate method is to identify the people and sources in the LLM-generated responses and then re-post the questions to those who have a reputation for having different views. For example, if the original answer came from a democratic right-leaning source, the prompt template may post the same question to a source of a republican-left persuasion, and vice versa. This approach allows for a more comprehensive examination of the topic by considering multiple perspectives.

The template to examine the semantic relation between two sentences $S_1$ and $S_2$ can be 
written as ``<$S_1$>, [R], [$S_2$],'' where R
is one of the three most important 
types of semantic relations: paraphrase, entailment, and contradiction \cite{PTRSUN2021}. Two sentences that have the same meaning are called paraphrases of each other. Two sentences that
have different meanings can be called 
disagreement or contradiction. The template 
can be trained to identify the degree
of agreement (or disagreement) between two
sentences.  


Table \ref{tab:Elenchus} shows two examples of this. In the first example (shown on the top portion of the table), the prompter asks GPT-3 to confirm if James Watson and Francis Crick are the only contributors to the discovery of the DNA double helix structure. GPT-3 replies by mentioning two other contributors. The second example in the table asks GPT-3 to provide not only the answer to a question but also its information sources and rate the credibility of each source according to the prompter's specification. Although the reliability of GPT-3's ratings remains to be validated, this rating mechanism can serve as an alert when some sources are found to be unreliable.


\begin{table}[htbp!]
\caption{Examples of Method Elenchus}
%\vspace{-.12in}
\label{tab:Elenchus}
%\resizebox{\textwidth}{!}
\begin{tikzpicture}
\begin{normalsize}
\node (table) [inner sep=0.1pt] {
\begin{tabular}{p{1.1cm}|p{6.4cm}}
\toprule
Role & Dialogue \\
\midrule
Prompt & {The discovery of the double helix structure of DNA was credited to James Watson and Francis Crick. However, are there opposing opinions to the list of contributors regarding this discovery?}\\

GPT3 & {There are some historical debates on the contributions of other scientists who also worked on the structure of DNA such as Maurice Wilkins and Rosalind Franklin.} \\ \\
\midrule 

Prompt & 
{What is the tallest building in the world.  Please provide three references and rate their credibility as high, medium, or low.} \\

GPT3 & {As of 2021, the tallest building in the world is the Burj Khalifa located in Dubai, United Arab Emirates. It stands at 828 meters (2,722 feet) tall.

References:
\begin{noindenumerate}
\item Credibility {\color{red}High}: "Burj Khalifa."... 
 this is the official website of the building, providing accurate information.
\item Credibility {\color{red}High}: "The Tallest Buildings in the World." Council on Tall Buildings and Urban Habitat... this is a well-respected organization in the field of tall building and urban habitat research.
\item Credibility {\color{red}Medium}: "The Tallest Buildings in the World." World Atlas..., 
this is a well-known website providing accurate information on different topics, but it's always good to cross-reference with other sources.
\end{noindenumerate}
}
%\bottomrule
\end{tabular}
};
\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
\end{normalsize}
\end{tikzpicture}
\end{table}


\subsection{Guided Generalization with Method Maieutics}

The example shown in Table~\ref{tab:Maieutics}, ``planting gourd yields cucumber,'' expects the GPT-3 to first learn to select the input objects are two produces, vegetables or fruit. The template is ``The farmer was so sad because he [verb] [X] but yields [Y], where price(X) >> price(Y).'' This first shot may not have strongly conveyed the condition: price(X) >> price(Y), but with a couple of training iterations, GPT-3 started to ``recognize'' the price constraint and could also provide justifications when arguing for the price of tea being much higher than the price of spinach (not presented in the table).
More interestingly, after GPT-3 gets the price right, it started suggesting food other than produce such as caviar, roe, lobster, and crab. While the price constraint was observed, the verb ``plant'' is incorrect. Here, we suggest making the hard-coded verb plant an output slot: ``The farmer was so sad because he [verb] [X] but yields [Y], where price(X) >> price(Y).''
Amazingly, GPT-3 is able to fill in with accurate verbs:
\begin{enumerate}
\item "Harvesting truffle yields mushroom."
\item "Fishing for caviar yields roe."
\item "Trapping lobster yields crab."
\end{enumerate}

The example shown in Table~\ref{tab:Maieutics}, ``planting gourd yields cucumber,'' demonstrates that GPT-3 is able to generate novel examples based on a template. When it suggests food items other than produce, it could be seen as an error as the boundary set by the verb ``plant'' is trespassed. However, this could also be seen as an innovative act by GPT-3, extending the constraint hinted by the verb. 
Impressively, the new examples still preserve the original intent of showing a producer's emotional distress.

How can this guided generalization be 
accurately and automatically
performed to edit a template?  
Socrates' method of generalization starts with specific instances and then draws general statements from them\footnote{The process of generalization in the Socratic method can be thought of as a form of induction, where specific examples are used to draw general conclusions. In the field of natural language processing and computational linguistics, there are a number of algorithms and techniques that have been proposed for identifying and extracting patterns from text data. These include methods for clustering, categorization, and classification of text data, as well as techniques for natural language understanding and information extraction. However, the specific algorithms and techniques used will depend on the specific task and application, and there is no one-size-fits-all procedure for generalization.}. The procedure for generalization involves identifying common patterns or themes in a set of examples, and then formulating a general rule that captures these patterns.
In the example presented in Table~\ref{tab:Maieutics},  we started with asking GPT-3 to meet the price(X) >> price(Y) constraint, with the condition that X and Y must both be produce grown in soil. However, upon analyzing GPT-3's outputs, we discovered that some instances of X and Y were not produce (e.g. lobster and caviar). This finding led to the realization that the hard-coded verb ``plant'' in the existing template was incorrect. To address this issue, generalization was applied by allowing the [verb] slot to be open, making the template statement more general. In this case, the mistakes made by GPT-3 served as valuable training data, allowing us to generalize the original template and make the expression more vivid and dynamic.


\subsection{Guided Imagination with Counterfactual}


Imagination and creating novel plots are crucial for writers, as it allows for ``creative freedom'' and ``artistic license.'' Creativity is the ability to think differently and approach problems with fresh and imaginative ideas.

However, an imagination without a clear subject matter, scope, or a story line can lead to a lack of productivity. To captivate the audience, a writer must consider human experiences and emotions as constraints. Therefore, ``creative freedom'' should not be viewed as total freedom, but rather as the ability to condition future narratives in the context and to create plots that turn and twist in unexpected ways.

The technique of counterfactual \cite{Pearl2009} can be useful in guiding imagination. It involves considering alternative scenarios and outcomes. This can lead to the exploration of different possibilities and the generation of new and unique plot ideas. For example, a writer may ask ``what if'' questions to change the narrative of events, such as ``what if the main character had not fallen in love?'' or ``what if an accident occurred on the way to a highly-anticipated date?'' By considering these counterfactuals, a writer and an LLM can create more engaging and interesting stories. One can ask an LLM to generate several scenarios and then select the most suitable one for the writer to continue writing.

As mentioned in Section~\ref{sec:cf}, we have experimented with using the counterfactual technique to
rewrite a chapter to connect the two greatest Chinese classical novels,
``Outlaws of the Marsh'' and ``Dream of the Red Chamber.'' We have
also asked GPT-3 to rewrite Genesis chapter 3 after verse six by prompting GPT-3
that: ``What if Adam and Eve refused the serpent to eat the fruit?''
The results were impressive, as GPT-3 was able to generate unique and interesting scenarios that deviated from the original story while still maintaining the core themes and concepts. 
This technique can be used in a wide range of writing and storytelling, 
from fiction to non-fiction, to generate new and compelling ideas. 

\subsection{Remarks on Evaluations}

Evaluating the strategies and methods presented in this section can be challenging as traditional methods such as using standard benchmarks may not be suitable for evaluating creative and imaginative output. Subjectivity can also play a role in the evaluation process. However, it is important to note that failure is a natural part of the writing process, as it often involves multiple revisions. In the specific case of our experiment in bridging two  classical novels, the process was a trial-and-error one with few successful ideas. However, there were two occasions where GPT-3 produced impressive results, which outweigh all the failures that occurred along the way for a writer.

==> MethodCounterfactual.tex <==
\subsection{Counterfactual Reasoning}
\label{sec:cf}

Counterfactual thinking refers to imaginative thoughts about what might have been (``if only'' or ``what if'').
Counterfactual reasoning can be useful in cross-examination~\cite{Cross-Examination2021,WinArgument2006} as it allows for the examination of what could have happened if a certain event or action did not occur. This can help to identify potential biases or limitations in the information being presented and can also provide alternative perspectives on the situation being examined.

For example, if a witness is testifying about an event that they observed, a counterfactual question could be used to ask what the witness would have observed if the event had occurred in a different way. This can help to identify any potential biases in the witness's testimony and can also provide a more comprehensive understanding of the event.

Additionally, the counterfactual technique can be used in cross-examination to test the robustness of the evidence and the strength of the argument presented by the witness. It can also be used to identify the assumptions that the argument is based on and to evaluate the plausibility of the alternatives proposed. Table~\ref{tab:WhatIf} presents an example of using the counterfactual technique during cross-examination to discredit a witness's testimony. 

\begin{table}[htbp]
\caption{An Example of Counterfactual Reasoning.}
%\vspace{-.12in}
\label{tab:WhatIf}
%\resizebox{\textwidth}{!}
\begin{tikzpicture}
\begin{normalsize}
\node (table) [inner sep=0pt] {
\begin{tabular}{p{1.2cm}|p{6.2cm}}
\toprule
Role & Dialogue \\
\midrule
Examiner & {Can you tell us what you saw on the night of the incident?} \\
Witness & {I saw the defendant break into the home.} \\
Examiner & {If the defendant had not been wearing a hat, would you have been able to identify him?} \\
Witness & {I'm not sure, it was dark and the at obscured his face. But I do remember his build and the way he walked.} \\
Examiner & {If the home had been equipped with better lighting, would you have been able to see the defendant's face?} \\

Witness & {Yes, I think I would have been able to see their face clearly.} \\

%\bottomrule
\end{tabular}
};
\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
\end{normalsize}
\end{tikzpicture}
%\vspace{-.1in}
\end{table}

We have experimented with using the counterfactual technique to rewrite a chapter to connect the two greatest Chinese classical novels, ``Outlaws of the Marsh'' and ``Dream of the Red Chamber.'' (The example is documented
in the extended version of this paper. The citation is removed for anonymous review.)
We have also asked GPT-3 to rewrite Genesis chapter 3 by 
prompting GPT-3 that: ``What if Adam and Eve refused the serpent to eat the fruit?''
Table~\ref{tab:genesis} in Appendix A presents GPT-3's 
creativity after our ``what if'' prompt.



==> MethodDefinition.tex <==
\subsection{Method of Definition}

The method of definition involves clarifying the meaning of key terms and concepts through a process of questioning. Through a cross-examination, it would involve asking questions to define the terms and concepts being discussed, to ensure that all parties have a common understanding of the subject at hand.


\begin{comment}
For example, in a legal cross-examination, the Socratic method could involve a lawyer questioning a witness about the meaning of certain key terms in their testimony, such as ``intent,'' ``negligence,'' or ``reasonable person.'' The lawyer may ask the witness to define these terms and provide examples to ensure that the witness has a clear understanding of the legal concepts relevant to the case. This helps to ensure that the testimony is clear, consistent, and relevant. Another example is when writing an essay on the subject of consciousness, one must first define the term consciousness and the scope of the discussion. The first response from an LLM may contain terminologies, such as awareness, attention, and unconsciousness, that require their definitions to be specified. If necessary,
the LLM can engage a dialogue with the
user to perform query refinement.
In short, the method of definition ensures that the prompter and the LLM are on the same page.
\end{comment}

==> MethodElenchus.tex <==
\subsection{Methods of Elenchus}

The name ``elenchus'' comes from the Greek word ``elenchein,'' which means to examine. 
The method of elenchus is often seen as a form of cross-examination \cite{Cross-Examination2021,WinArgument2006}, in which a teacher uses questions and counter-questions to expose contradictions and inconsistencies in a student's beliefs and attitudes, in order to arrive at a deeper understanding of a topic.

An example of the method of elenchus in action would be a dialogue between Socrates and a student in which Socrates asks a series of questions to help the student understand the concept of justice. For example, Socrates might ask the student to define justice, and then ask follow-up questions to expose any contradictions or inconsistencies in the student's definition. Through this process of questioning and counter-questioning, Socrates aims to help the student arrive at a deeper understanding of justice.

\begin{comment}
How do we design a prompt template for these methods?
When utilizing these methods in a dialogue with a language model, the primary focus is on identifying and addressing inconsistencies. This can be done by following a process similar to legal cross-examination, first establishing the credibility of the language model's sources, identifying and addressing inconsistencies of multiple sources (witnesses), and highlighting key points that support the conclusions \cite{}.

It is important to note that a language model can produce biased or incorrect answers. To ensure the credibility of the answers, it can be helpful to ask the language model for its sources of information and then validate the credibility of those sources. By having multiple answers, their information sources, and the credibility of those sources, a more trustworthy answer can be derived.
\end{comment}

\begin{table}[htbp!]
\caption{Identifying Inconsistency (ChatGPT 1/23/2023)}
\label{tab-lake}
%\resizebox{\textwidth}{!}
\begin{tikzpicture}
\begin{normalsize}
\node (table) [inner sep=0pt] {
\begin{tabular}{p{1.1cm}|p{6.2cm}}
\toprule
Role & Dialogue \\
\midrule
Prompt & {What is the third largest lake in the world?} \\
GPT3 & {The third largest lake in the world is Lake Superior. } \\
Prompt & {What are the five largest lakes in the world?} \\
GPT3 & {They are:
1) Caspian Sea, 2) Superior, 3) Victoria,
4) Huron, 5) Michigan.
} \\
Prompt & {Your two answers contradict. You first answered me Lake Superior is the third largest lake, but your top five list shows Victoria is the third, and Superior is the second largest lake.} \\
GPT3 & {I apologize for the confusion. Lake Superior is indeed the largest lake in the world by area, but it is not considered a lake by some geographers because it is part of the Great Lakes system, which is connected to the Atlantic Ocean via the St. Lawrence River. In terms of the top ten largest lakes in the world, Lake Victoria is considered the third largest lake by area. My apologies for any confusion caused.} \\
%\bottomrule
\end{tabular}
};
\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
\end{normalsize}
\end{tikzpicture}
\vspace{-.1in}
\end{table}
\hfill \break
\noindent
{\bf Example}: {\em What is the third largest lake in the world?}
%\subsubsection*{Example: What is the third largest lake in the world?}
\hfill \break
Figure~\ref{tab-lake} presents an example prompting session with ChatGPT.  The first prompt queries ChatGPT for the third largest lake in the world.  ChatGPT returns ``Lake Superior.''  The second prompt asks for the ten largest lakes, on which the thrid largest is ``Lake Victoria.''  After pointing out the inconsistency to ChatGPT, it returns that ``Lake Victoria'' is the right answer to the first prompt, and it also provides the reason for its mistake.
(We tested on ``the fifth highest mountain in the world'' and went through a similar consistency check, and the answer provided by ChatGPT is accurate.)

%Depending on the importance of the answer, a prompt template may want to identify three or more reliable sources and then query LLMs for both answers and references. A credential check on references is similar to a credential check on a witness in a legal proceeding. 


==> MethodHypothesis.tex <==
\subsection{Method Hypothesis Elimination}

The Socratic method is a process of identifying and eliminating false hypotheses through a series of logical and factual questions. It aims to uncover commonly held truths and test their consistency with other beliefs. The method is based on asking questions to explore definitions and identify the general characteristics shared by different instances.

When utilizing the method of hypothesis elimination in a dialogue with a language model, the primary focus is on identifying and addressing inconsistencies. One way to achieve this is by creating a prompt template that is specifically designed to uncover inconsistencies. This can be done by following a process similar to legal cross-examination, first establishing the credibility of the language model's sources, identifying and addressing inconsistencies of multiple sources (witnesses), and highlighting key points that support the conclusions \cite{}.

It is important to note that language models can produce biased or incorrect answers. To ensure the credibility of the answers, it can be helpful to ask the language model for its sources of information and then validate the credibility of those sources. By having multiple answers, their sources, and the credibility of those sources, a more trustworthy answer can be derived.

\subsubsection{Example \#1: What is the third largest lake in the world?}

\begin{table}[ht!]
\caption{What is the third largest lake in the world? (ChatGPT 1/23/2023)}
\label{tab-lake}
%\resizebox{\textwidth}{!}
\begin{tikzpicture}
\begin{small}
\node (table) [inner sep=0pt] {
\begin{tabular}{p{1.2cm}|p{6.6cm}}
\toprule
Role & Dialogue \\
\midrule
Prompt & {What is the third largest lake in the world?} \\
GPT3 & {The third largest lake in the world is Lake Superior. } \\
Prompt & {What are the ten largest lakes in the world?} \\
GPT3 & {They are:
\begin{noindenumerate}
\item Caspian Sea
\item Superior
\item Victoria
\item Huron
\item Michigan
\item ...
\end{noindenumerate} \\
Prompt & {Your two answers contradict. You first answered me Lake Superior is the third largest lake, but your top ten list shows Victoria is the third, and Superior is the second largest lake.} \\
GPT3 & {I apologize for the confusion. Lake Superior is indeed the largest lake in the world by area, but it is not considered a lake by some geographers because it is part of the Great Lakes system, which is connected to the Atlantic Ocean via the St. Lawrence River. In terms of the top ten largest lakes in the world, Lake Victoria is considered the third largest lake by area. My apologies for any confusion caused.} \\
} \\
%\bottomrule
\end{tabular}
};
\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
\end{small}
\end{tikzpicture}
\end{table}

Table~\ref{tab-lake} presents an example prmpting session with ChatGPT, performed on January 19th, 2023.  The first prompt queries ChatGPT for the third largest lake in the world.  ChatGPT returns ``Lake Superior.''  The second prompt asks for the ten largest lakes, on which the thrid largest is ``Lake Victoria.''  After pointing out the inconsistency to ChatGPT, it returns that ``Lake Victoria'' is the right answer to the first prompt, and it also provides the reason for its mistake.
(We tested on ``the fifth highest mountain in the world'' and went through a similar consistency check, and the answer provided by ChatGPT is accurate.)

Depending on the importance of the answer, a prompt template may want to identify three or more reliable sources and then query LLMs for both answers and references. A credential check on references is similar to a credential check on a witness in a legal proceeding. 



==> MethodMaieutics.tex <==
\subsection{Method of Maieutics}
\label{sec:Maieutics}

The term ``maieutic'' comes from the Greek word ``maieutikos,'' which means midwife. The maieutic method is based on the premise that a teacher's role is to assist students in giving birth to their own understanding of a subject, rather than simply conveying knowledge. Unlike the elenctic method, which aims to identify and eliminate false hypotheses, maieutics centers on helping students reveal their own understanding of a subject. This dialogical method involves the teacher asking questions designed to aid the student in discovering their own comprehension, rather than providing answers or information.


\hfill \break
\noindent
{\bf Example}: {\it From being ignorant to creative.}
%\subsubsection*{Example: From being ignorant to creative using method maieutics.}
\hfill \break
We use the example in Table~\ref{tab:Maieutics} to illustrate how GPT-3 starts from knowing nothing about the semantics of an idiom to being able to create new idioms expressing the same meaning with different metaphors. Initially, GPT-3 did not have a clear understanding of the Taiwanese idiom: ``planting gourd yields cucumber.'' The idiom conveys the meaning that when a farmer plants gourds, which are more valuable and have a higher market price, but unexpectedly harvests cucumbers, which have a lower market price, the farmer not only experiences disappointment but also suffers from financial loss.
GPT-3 initially could not understand the full meaning of the idiom.  After a couple of iterations, GPT-3 ``gives birth'' impressive new variations. 

\begin{table}[htbp]
\caption{Example of Method Maieutics}
%\vspace{-.1in}
\label{tab:Maieutics}
%\resizebox{\textwidth}{!}
\begin{tikzpicture}
\begin{small}
\node (table) [inner sep=0pt] {
\begin{tabular}{p{1.2cm}|p{6.5cm}}
\toprule
Role & Dialogue \\
\midrule
Prompt & {Can you interpret the meaning of this Taiwanese idiom: "planting gourd yields cucumber?"}\\
GPT3 & {The idiom is often used to convey the idea that sometimes, despite your best efforts, things don't turn out the way you want them to..} \\
Prompt & {You are half right. It also implies that the price of gourd is much higher than the market price of cucumber. The farmer not only yields unexpected results, but also loses income! } \\

GPT3 & {It's an idiomatic expression that can be used to describe a situation in which someone works hard and invests a lot of resources into something, but the outcome is not only different from what was expected, but also less profitable. It conveys the idea of frustration and financial loss.} \\

Prompt & {Can you replace the two vegetables, gourd and cucumber, with two other plants and still maintain the meaning of the idiom?} \\

GPT3 & {These are three examples:
\begin{noindenumerate}
\item "Planting strawberry yields raspberry," which
conveys the idea of disappointment and financial loss when someone plants more valuable and expensive strawberry but ends up getting less valuable and cheaper raspberry.
\item "Planting melon yields watermelon."...
\item "Planting apple yields pear."...
\end{noindenumerate}
} \\
Prompt & {In your examples, your two vegetables or fruits are similar in price.  Please consider price when
formulating your idioms.} \\

GPT3 & {I apologize. These are three new examples:
\begin{noindenumerate}
\item "Planting truffle yields mushroom."...
\item "Planting caviar yields roe."...
\item "Planting lobster yields crab."...
\end{noindenumerate}
} \\
Prompt & {Great! In these examples you did consider values of the objects. But do you know that lobster and crab are not plants. They are both phylum arthropods and they live in water. They cannot be planted! }  \\

GPT3 & {... I apologize... Lobster and crab are not plants, and they cannot be planted. They are both members of the phylum arthropoda, and live in water. Instead of ``planting,'' verbs should be appropriate for these animals, such as:
\begin{noindenumerate}
\item "Planting truffle yields mushroom."...
\item "Harvesting caviar yields roe."...
\item "Catching lobster yields crab."...
\end{noindenumerate}
}
%\bottomrule
\end{tabular}
};
\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
\end{small}
\end{tikzpicture}
%\vspace{-.1in}
\end{table}


==> PilotStudy.tex <==
\section{Pilot Study}
\label{sec:pilot}

Our pilot study uses CRIT, and it aims to answer two questions:
Should all prompts be issued to GPT-3 sequentially or they
can be issued all together?  
What limitations can be identified for improvement?
The study utilizes exercises with established answers from the $8^{th}$ edition of the textbook ``Ask the Right Questions'' by the authors of \cite{AskRightQ2001}. It is important to note that the study evaluates the effectiveness of CRIT's prompt template, rather than the language models to which CRIT can issue prompts.

\begin{comment}
Table~\ref{tab:pilot1} presents two examples from \cite{AskRightQ2001}. The results of the CRIT analysis, which include conclusion extraction and reason identification, match or exceed the evaluations made by the authors. In the first example, the authors consider the document to be somewhat ambiguous with two potential conclusions. CRIT finds the document to be poorly written without a clear conclusion and gives it a low validity score of $60\%$. This low credibility score is attributed to the absence of sufficient evidence in the argument to justify two possible claims. 
In the second example, CRIT accurately extracts the claim and arguments and recognizes that the argument's validity is subjective and dependent on context such as religious beliefs and cultural perspectives. 
\end{comment}

On short documents, the results are similar in quality when CRIT is used to issue prompts either sequentially or all together as one prompt, as long as the instructions are consistent. However, when evaluating long articles in \cite{501Q2004}, CRIT issuing prompts one after another yields much higher presentation quality in both organization and clarity. 
(Due to the space limit, we document examples in a supplement document \cite{CRITExtended2023}.) In the teaching mode, the sequential option is thus much preferred. Furthermore,
When a reason is itself a claim and requires CRIT to validate its supporting references, using a sequential approach is more flexible and enables CRIT to query for references and then execute the process recursively.

\begin{table}[hbt!]
%\vspace{-.1in}
%\resizebox{\textwidth}{!}
\begin{tikzpicture}
\begin{small}
\node (table) [inner sep=0pt] {
\begin{tabular}{p{0.8cm}|p{6.6cm}}
\toprule
\textbf{Role} & \textbf{Dialogue} \\
\midrule
{Input} & {When cases increase and transmission accelerates, it’s more likely that new dangerous and more transmissible variants emerge, which can spread more easily or cause more severe illness.

Based on what we know so far, vaccines are proving effective against existing variants, especially at preventing severe disease, hospitalization and death. However, some variants are having a slight impact on the ability of vaccines to guard against mild disease and infection.

Vaccines are likely staying effective against variants because of the broad immune response they cause, which means that virus changes or mutations are unlikely to make vaccines completely ineffective.} \\

{CRIT} & {[Conclusion]: Vaccines are effective at preventing severe disease, hospitalization and death, and likely will remain effective against variants due to the broad immune response they cause.} \\

& [Reasons]: Four reasons listed are: \\
& 1.  Cases increase and transmission accelerates leads to emergence of new dangerous and more transmissible variants. \\
& 2. Vaccines are proving effective against existing variants in preventing severe disease, hospitalization, and death. \\
& 3. Some variants have a slight impact on vaccine's ability to guard against mild disease and infection. \\
& 4. Broad immune response caused by vaccines make virus changes or mutations unlikely to make vaccines completely ineffective. \\
\midrule
{$\Gamma$ score} & {[{\color{red}8/10}] Validity of argument: 8/10. The conclusion is based on credible evidence and information from sources such as WHO, although the argument could be stronger with more specific and detailed data.} \\
& {[{\color{red}9/10}] Sources credibility: 9/10. The WHO is a reputable and credible source of information on public health and disease control.} \\
%\textbf{Final Score}: {\color{red}$72\%$ High} (High: above $60\%$, Low: below $25\%$)
%$} \\
\bottomrule
\end{tabular}
};
\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
\end{small}
\end{tikzpicture}
%\vspace{-.05in}
\caption{Pilot Study on CRIT. 
%WHO's post about the expected efficacy of 
%COVID vaccines on its variants.
}
\vspace{-.20in}
\label{tab:pilot2}
\end{table}

Table~\ref{tab:pilot2} presents a document about COVID-19 vaccine efficacy, published by the World Health Organization (WHO) in July 2021 on its homepage \cite{WHO2021}. The article remains available on the WHO's website, indicating that its information is still considered valid by the organization. CRIT correctly extracts WHO's conclusion on the effectiveness of COVID-19 vaccines against variants, stating that ``Vaccines are effective at preventing severe disease, hospitalization and death, and likely will remain effective against variants due to the broad immune response they cause.'' This conclusion is supported by four strong arguments. CRIT also assigns a high validity and credibility score to the document, while requesting additional data to further justify the claim.




